A Generic Model of Contracts for Embedded Systems

We present the mathematical foundations of the contract-based model developed in the framework of the SPEEDS project. SPEEDS aims at developing methods and tools to support "speculative design", a design methodology in which distributed designers develop different aspects of the overall system, in a concurrent but controlled way. Our generic mathematical model of contract supports this style of development. This is achieved by focusing on behaviors, by supporting the notion of "rich component" where diverse (functional and non-functional) aspects of the system can be considered and combined, by representing rich components via their set of associated contracts, and by formalizing the whole process of component composition.

==> contract.tex <==
\section{Rich Components and Assume/Guarantee
reasoning}\label{sec:contracts}
\newcommand{\pre}{{\it pre}}
\newcommand{\tle}{{\rm TLE}}
\newcommand{\never}{{\it never}}
\newcommand{\always}{{\it always}}


\subsection{Heterogeneous Rich Components}\label{sec:hrc}
The main element of our semantic model is a \emph{Heterogeneous Rich
Component}, or simply a component.
A component is composed of an \emph{interface}, its \emph{expected
behavior}, and, optionally, of one or more \emph{implementations}.
The interface of a component consists of a set of ports and flows, which are
used by the component to communicate with the rest of the system and with
the environment.
The expected behavior is instead described by one or several
\emph{assumption}/\emph{promise} pairs, called \emph{contracts}.
Contracts can be combined together using three composition operators:
greatest lower bound, parallel composition and fusion.
The greatest lower bound is used to compose contracts referring to the same
component and which use only variables and flows visible from the
environment.
Parallel composition is used to compute the contract resulting from the
composition of several components.
Fusion generalizes these two operators, and is capable of handling all
cases.
In particular, it is used to compose contracts whenever the greatest lower
bound and parallel composition operators are inappropriate, for instance
when contracts share local variables or flows.
Thus, fusion is the implicit composition of contracts, whenever more than
one contract is attached to a component.
Implementations may be attached to a component, and are usually expressed as
extended state machines, or as host tool models.

We define several relations between components, contracts and
implementations.
\begin{itemize}
  \item The \emph{compatibility} relation relates sets of components.
    It is easier to define the negation of compatibility: A set of
    components are \emph{incompatible} whenever for all environments, at
    least one of the assumption of at least one component is violated.
    This means that in a compatible set of components, the assumption
    resulting from the parallel composition of component contracts is
    universal, i.e., all assumptions required for the correct behavior
    of the system have been discharged.
  \item Contract \emph{dominance} relates assumptions and promises of two
    contracts.
    Contract $\cgte = (\assp, \prom)$ dominates contract $\cgte' = (\assp',
    \prom')$ whenever $\assp' \subseteq \assp$ and $\prom \subseteq \prom'$.
  \item \emph{Satisfaction} relates implementations to contracts.
    An implementation $\comp$ satisfies contract $\cgte = (\assp ,\prom)$
    whenever $\comp \intersect \assp \subseteq \prom$.
  \item \emph{Refinement} relates implementations.  Implementation $\comp$
    refines implementation $\comp'$ whenever $\comp \subseteq \comp'$.
\end{itemize}
%
% In this section we 
We are now ready to formalize our contract based approach. The two
central notions are \emph{implementations} and \emph{contracts},
whereas \emph{rich components} will provide the needed syntactic
framework for our component based design methodology.

In a first subsection we discuss assume/guarantee reasoning without
considering the issue of splitting of responsibilities among
concurrent designers. 
%
In a second subsection, we refine our theory of contracts by
considering the splitting of responsibilities among concurrent
designers. This is achieved by splitting sets of ports, variables, and
parameters into controlled and uncontrolled ones, from the perspective
of a given designer. In specifying promises of a contract, or going
for an implementation, this designer will be allowed to constrain only
the ports and variables she/he controls.

Throughout this section we shall need an abstract notion of ``assertion''.
For the moment, the only facts we need to know about assertions can be 
summarized as follows:
\begin{itemize}
\item Each assertion $\behav$ possesses a set of \emph{ports} and a set of
  \emph{variables} that are the vehicle for interaction.
\item An assertion is identified with the set of runs it defines or accepts.
  A run assigns a history to each variable and ports of the assertion.
  We assume that a proper notion of ``complement'' for an assertion $\behav$
  is available, we denote it by $\complement{\behav}$.
\item When seen as sets of runs, assertions compose by intersection --- note
  that such an operation is monotonic w.r.t.\ inclusion of sets of runs.
  When performing this composition or product, we assume that the
  appropriate inverse projections have been performed to equalize the
  involved sets of ports and variables.
  Products are equivalently denoted by $\behav_1 \times \behav_2$ or
  $\behav_1 \cap \behav_2$.
\end{itemize}

\subsection{Rich Components, Contracts, and Implementations}
\begin{definition}[Implementation] \label {erpwifuerilu}
An \emph{implementation} is simply an assertion, that is, a set of runs.
\end{definition}
We use the symbol $\comp$ to generically refer to implementations
(symbol $\comp$ is reminiscent from ``machine'').  Implementations are
ordered according to the runs they contain.  An implementation $\comp$
\emph{refines} an implementation $\comp'$, written $\comp \compref
\comp'$ if and only if $\comp$ and $\comp'$ are defined over the same
set of ports and variables, and
\[
\comp \subseteq \comp'.
\]
Products preserve implementation refinement.

A \emph{\contract} says that under certain assumptions, behaviors are
guaranteed to be confined within a certain set.

\begin{definition}[{\Contract}]\label{def:contract}
A \emph{\contract} $\cgte$ is a pair $(\assp, \prom)$, where $\assp$,  the
\emph{assumption,} and $\prom$, the \emph{promise,} are assertions over the
same alphabet.
Whenever convenient, we shall denote by $\assp_\cgte$ and $\prom_\cgte$ 
the assumption and promise of contract $\cgte$.
\end{definition}
%
The interpretation of a {\contract} is made precise by the following
definition.
\begin{definition}[Satisfaction]\label{def:satisfaction}
An implementation $\comp$ satisfies a {\contract} $\cgte = (\assp, \prom)$, written
$\comp \models \cgte$, if and only if
\[
\comp \intersect \assp \subseteq \prom.
\]
\end{definition}
Satisfaction can be checked using the following equivalent formulas, where
$\complement{\assp}$ denotes the set of all runs that are not runs of $\assp$:
%
\begin{eqnarray}
\comp \models \cgte \ \iff \ \comp \subseteq \prom \union \complement{\assp}
\ \iff \ \comp \intersect (\assp \intersect \complement{\prom}) = \emptyset
\label{th:alt_satisfaction}
\end{eqnarray}
%
There exists a unique maximal implementation satisfying a contract 
$\cgte$, namely: 
%
\beq
\maxcomp{\cgte} &=& G \cup \complement{\assp}
\label {'eotj[i}
\eeq
%
\begin{definition}[Rich Component] \label {epfiueipu}
A \emph{rich component} is a tuple 
%
\beq
\richcomp &=& \bigl(\rcname, \setsofcontracts, \optimplementation\bigr)
\label {epruifgeipu}
\eeq
%
In (\ref{epruifgeipu}), $\rcname$ is the \emph{name} of the rich
component, $\setsofcontracts$ is a (possibly empty) set of contracts,
and $\optimplementation$ is an (optional) implementation such that
$\optimplementation\models\setsofcontracts$, where the meaning of the
latter property is postponed to Definition \ref{pweifugbepruif}.
\end{definition}
%
Note that the concept of rich component is purely syntactic, since it
only consists in giving a name to a tuple composed of a set of
contracts together with an optional implementation of it. We shall
therefore mainly focus in the sequel on contracts and implementations.

\paragraph*{Canonical forms}
Note that $\maxcomp{\cgte}$ is to be interpreted as the implication
$\assp\Rightarrow\prom$. We have that $\comp\models(\assp,\prom)$, if
and only if $\comp\models(\assp,\maxcomp{\cgte})$, if and only if
$\comp\subseteq\maxcomp{\cgte}$.  Say that contract $\cgte = (\assp,
\prom)$ is in \emph{canonical form} when $\prom = \maxcomp{\cgte}$,
or, equivalently, when $\complement{\assp}\subseteq\prom$
or  when $\complement{\prom}\subseteq\assp$. Thus, every
{\contract} has an equivalent {\contract} in canonical form, which can
be obtained by replacing $\prom$ with $\maxcomp{\cgte}$.  Hence,
working with {\contracts} in canonical form does not limit
expressiveness.  The operation of computing the canonical form is well
defined, since the maximal implementation is unique, and it is
idempotent.
%
\beq\bea{l}
\mbox{\emph{In the following, we assume that}}
\\
\mbox{\emph{all {\contracts} are in canonical form.}}
\eea
\label {erotihjpui}
\eeq
% 
\begin{example}{Running example: control/monitoring unit}
\label {rfguioerhfui}
%
%
%
Throughout this paper, we develop the system of Figure~\ref{erpfiuerhpifu}
to illustrate our notion of contract and its use. It consists
of a control unit interacting with a monitoring unit.
% The system is
% synchronous in that both components are triggered by the same periodic
% clock.  This system is subject to two independent faults, $f_1$ for
% the control unit, and $f_2$ for the monitoring unit. To simplify we
% assume that faults are permanent, i.e., once they occurred, they are
% active for ever.
\begin{figure}[h]
\centerline{\input{monitoring0.pstex_t}}
\caption[kuyf]{\small Running example: control/monitoring system.}
\label {erpfiuerhpifu}
\end{figure}
% Since the system involves no delay, we can forget about time and dynamics 
% and regard it as simple propositions.

The nominal behaviour of the system (when $f_1=\false$) is that
it should deliver $y=a\wedge b$ at its output. When safe
($f_2=\false$), the monitoring unit ensures that, if the control unit
gets faulty ($f_1=\true$), the overall system is shut down
($y=\false$) unless $a=\true$ holds. Thus the Top Level Exception
(TLE) is equal to $\tle=\neg a \wedge y$.  This TLE may, however, get
violated if the monitoring unit gets faulty too ($f_2=\true$).
%
These requirements are summarized by the two contracts
$\cgte$, for the nominal mode, and $\cgte'$ for the exception mode:
%
\beq\bea{rclcl}
\cgte &=& (\,\neg f_1\,,\,y=a\wedge b\,) &:&\mbox{nominal mode}
\\
\cgte' &=& (\,\neg f_2\,,\,\neg\tle\,) &:&\mbox{exception mode}
\\
\tle &=&\neg a \wedge y &:& \mbox{top level exception}
\eea
\label {rpefuiehpu}
\eeq
%
This separation of concerns into nominal and exception mode is very
similar to the separation of viewpoints (e.g., functional,
timed, safety, etc) in handling components via their contracts.
\end{example}

\subsection{Operations on contracts}
\subsubsection{Boolean algebra on contracts}
As usual, it will be useful to have a ``logic'' providing ways of
expressing more complex contracts from simpler ones. The following
relation of dominance formalizes substituability for contracts, it
induces a boolean algebra of contracts, which provides such a logic of
contracts. 

\begin{definition}[Dominance]\label{def:dominance_restricted}
Say that {\contract} $\cgte = (\assp, \prom)$ dominates 
{\contract} \mbox{$\cgte' = (\assp', \prom')$,} written $\cgte \cgref
\cgte'$, if and only if $\assp \supseteq \assp'$ and $\prom \subseteq
\prom'$.
\end{definition}
Dominance amounts to relaxing assumptions and reinforcing
promises. Note that $\cgte \cgref \cgte'$ and $\cgte' \cgref \cgte$
together imply $\cgte = \cgte'$.  Furthermore,
%
\beq
\cgte \cgref \cgte' &\implies& \maxcomp{\cgte} \models \cgte'
\label {erpotgihpeori}
\eeq
%
but the converse is not true. Property (\ref{erpotgihpeori}) implies
the following result:
\begin{lemma} \label {erpifugefipu}
If $\comp\models\cgte$ and $\cgte\cgref\cgte'$, then $\comp\models\cgte'$.
\end{lemma}
The following theorem defines a boolean algebra
over contracts. Its proof is straightforward and left to the reader.

%
\begin{theorem} [Boolean algebra of contracts] 
\label {th:bounds_restr}
Let $\cgte_1 = (\assp_1, \prom_1)$ and $\cgte_2 = (\assp_2, \prom_2)$
be {\contracts}.  Then, the greatest lower bound of $\cgte_1$ and
$\cgte_2$, written $\cgte = \cgte_1 \meet \cgte_2$, is given by $\cgte
= (\assp, \prom)$ where $\assp = \assp_1 \union \assp_2$ and $\prom =
\prom_1 \intersect \prom_2$. Note that the so defined pair
$(\assp,\prom)$ is in canonical form.

Similarly, the least upper bound of $\cgte_1$ and $\cgte_2$, written
$\cgte = \cgte_1 \join \cgte_2$, is given by $\cgte' = (\assp',
\prom')$ where $\assp = \assp_1 \intersect \assp_2 $ and $\prom =
\prom_1 \union \prom_2 $. Note that the so defined pair
$(\assp,\prom)$ is in canonical form.

The minimal and maximal contracts are $\bot=(\runs, \emptyset)$ and
$\top=(\emptyset, \runs)$, respectively, where $\runs$ denotes the set of
all runs.

Finally, the complement of $\cgte$ is the {\contract}
$\complement{\cgte}$ such that $\complement{\cgte} =
(\complement{\assp}, \complement{\prom}) $; it satisfies 
$\complement{\cgte}\meet\cgte=\bot$ and 
$\complement{\cgte}\join\cgte=\top$.
\end{theorem} 

\begin{example}{Running example cont'd: greatest lower bound}
\label {e;rouifhe}
The two contracts of (\ref{rpefuiehpu}) represent two viewpoints
attached to a same component, corresponding to the nominal and
exception modes, respectively. These two contracts involve the same
set of ports.  Combining them is by computing their greatest lower
bound.  Putting these two contracts in canonical form and then taking
their greatest lower bound yields:
% fusing them yields the equivalent global contract:
%
\beqq
\cgte \;\meet\; \cgte'
= \left(\,\neg (f_1\wedge f_2)\,,\,
% \neg (f_1\wedge f_2)\Ra
\left[\bea{cl}
& \neg f_1 \Ra y=a\wedge b
\\
\wedge & \\
& \neg f_2 \Ra \neg 
\tle\eea\right]\,\right)
\eeqq
%
This contract assumes that no double failure occurs. Its promise is
the conjunction of the promises of $\cgte$ and $\cgte'$.  Expanding
the promise of this global contract leads to a cumbersome formula,
hardly understandable to the user, so we discard it.
\end{example}

\subsubsection{Parallel composition}
Contract composition formalizes how contracts attached to different
rich components should be combined to represent a single, compound,
rich component.
%
Let $\cgte_1 = (\assp_1, \prom_1)$ and $\cgte_2 = (\assp_2, \prom_2)$ be
{\contracts}.
First, composing these two contracts amounts to composing their promises.
Regarding assumptions, however, the situation is more subtle.
Suppose first that these two contracts possess disjoint sets of ports and
variables.
%
% Then, the assumptions of the composite is intuitively simply the
% conjunction of the assumptions of the components, since the
% environment should satisfy all the assumptions.\footnote{This is not
% quite true in our definition of composition.  However, the projection
% of the resulting assumptions on the alphabet of the components is
% equal to the assumptions of the components, so effectively all
% assumptions are retained.}
At a first sight, the assumptions of the composite should intuitively
be simply the conjunction of the assumptions of the rich components,
since the environment should satisfy all the assumptions.
%
In general, however, part of the assumptions $\assp_1$ will be already
satisfied by composing $\cgte_1$ with $\cgte_2$, acting as a partial
environment for $\cgte_1$.
Therefore, $\prom_2$ can contribute to relaxing the assumptions $\assp_1$.
And vice-versa.
Whence the following definition:

\begin{definition}[Parallel composition of contracts]
\label{def:composition_restr}
Let $\cgte_1 = (\assp_1, \prom_1)$ and $\cgte_2 = (\assp_2, \prom_2)$
be {\contracts}. Define $\cgte_1 \product \cgte_2$ to be the contract
$\cgte = (\assp, \prom)$ such that:
\begin{eqnarray*}
\assp & = & (\assp_1 \intersect \assp_2) \union \complement{(\prom_1
\intersect \prom_2)}, \\
\prom & = & \prom_1 \intersect \prom_2.
\end{eqnarray*}
Note that the so defined contract is in canonical form.
\end{definition}
The following result expresses the compositionality of implementation
relation:
\begin{lemma} \label {oeifuygrui}
$\comp_1\models\cgte_1$ and $\comp_2\models\cgte_2$ together 
imply \mbox{$\comp_1\times\comp_2 \;\models\; \cgte_1 \product \cgte_2$.}
\end{lemma}
\begin{proof}
The assumption of the lemma means that
$\comp_i\subseteq\maxcomp{\cgte_i}$, for $i=1,2$. Since the two
contracts are in canonical form, we have $\maxcomp{\cgte_i}=\prom_i$
and the result follows directly from Definition \ref{def:composition_restr}.
\end{proof}
The following lemma relates greatest lower bound and parallel
composition, it relies on the fact that we work with contracts in
canonical form:
\begin{lemma} \label {wrotheortui}
For any two contracts, % $\cgte_1$ and $\cgte_2$, % ,i=1,2$, we have 
$\cgte_1\meet\cgte_2 \cgref \cgte_1\para\cgte_2$.
\end{lemma} 
\begin{proof}
Both sides of this relation possess identical promises. Thus the only
thing to prove relates to the assumptions thereof.  From
Definition~\ref{def:composition_restr} and
Theorem~\ref{th:bounds_restr}, the assumption of $\cgte_1\meet\cgte_2$
is equal to $\assp_1\cup\assp_2$, whereas the assumption of
$\cgte_1\para\cgte_2$ is equal to $(\assp_1 \intersect \assp_2) \union
\complement{(\prom_1 \intersect \prom_2)}$. Since the two contracts
are in canonical form, we have $\complement{\prom_i}\subseteq\assp_i,
i=1,2$, and thus $\complement{(\prom_1\cap\prom_2)}
=\complement{\prom_1}\cup\complement{\prom_2}
\subseteq\assp_1\cup\assp_2$. Therefore, the assumption of
$\cgte_1\para\cgte_2$ is contained in $\assp_1\cup\assp_2$, which is
the assumption of $\cgte_1\meet\cgte_2$. This proves the lemma.
\end{proof}
%
\begin{example}{Running example cont'd: compositional reasoning}
\label {;erfouihe;uio}
In Example~\ref{e;rouifhe}, we have shown how to combine the two
nominal and exception viewpoints, for the overall system of
Figure~\ref{erpfiuerhpifu}. But this system itself decomposes into its
control and monitoring unit. We would like to associate contracts to
each of these components, for each of their viewpoint. And we would
like to be able to compose the resulting contracts, and, by doing so,
recover the system overall contract.

Since the overall system is the parallel composition of control and
monitoring units, then we may reasonably expect that the parallel
composition of contracts, for each of these components, should be
used. However, we are also combining viewpoints for these two
components and we have seen that this sould be performed by using the
greatest lower bound. So, which one is the correct answer?

Actually, none of them, as we shall see. The new notion of contract
\emph{fusion} we shall introduce in the following section, will
provided the adequate answer. Prior to introduce this notion, we need
to investigate what it means to eliminate ports in contracts.
\end{example}


\subsubsection{Eliminating ports in contracts}
Elimination in contracts requires handling assumptions and promises
differently.
%
\begin{definition} [Elimination]
\label {erotijherio}
Let $\cgte=(\assp,\prom)$ be a contract 
% defined over a set of ports $P_\cgte$, 
and let $p$ be any port. Define the \emph{elimination of $p$
in $\cgte$ by:} 
%
\beqq 
\elim{\cgte}{p} &=& (\forall p \,\assp, \exists p \,
\prom) 
\eeqq
%
where $\assp$ and $\prom$ are seen as predicates.
\end{definition}
Note that we do not require that $p$ be a port of $\cgte$.
Definition~\ref{erotijherio} is motivated by the following lemma:
%
\begin{lemma}\label{erptihpui}
We have $\cgte\cgref\elim{\cgte}{p}$. Furthermore, let $\comp$ be an
implementation such that $\comp\models\cgte$ and $p$ is not a port of
$\comp$.  Then, $\comp\models\elim{\cgte}{p}$.
\end{lemma}
\begin{proof}
This result does not require that $\cgte$ is in canonical form. 
Condition $\comp\models\cgte$ is
equivalent to $\comp\cap\assp\subseteq\prom$. Eliminating $p$, with
$\forall$ on the left hand side and $\exists$ on the right hand side,
yields $[\forall p\,(\comp\cap\assp)]\subseteq[\exists p\,\prom]$ and
the lemma follows from the fact that $\forall p\,(\comp\cap\assp)
=\comp\cap(\forall p\,\assp)$ if $p$ is not a port of $\comp$.
\end{proof}
%
The following lemma relates elimination and greatest lower bounds:
%
%\clearpage
\begin{lemma}  \label {erptfuhpeioru}
For any two contracts $\cgte_1$ and $\cgte_2$ and any port $p$, we have
%
\beq
\elim{\cgte_1 \meet \cgte_2}{p} 
&\cgref&
\elim{\cgte_1}{p} \meet \elim{\cgte_2}{p} 
\label {we;rofh;sro}
\\
\elim{\cgte_1 \para \cgte_2}{p} 
&\cgref&
\elim{\cgte_1}{p} \para \elim{\cgte_2}{p} 
\label {erptheruih}
\eeq
\end{lemma}
\begin{proof}
We have $\forall p\,(\assp_1\cup\assp_2)\supseteq(\forall
p\,\assp_1\cup\forall p\,\assp_2)$ and $\exists
p\,(\prom_1\cap\prom_2)\subseteq$ \mbox{$(\exists
p\,\prom_1\cap\exists p\,\prom_2)$,} which proves (\ref{we;rofh;sro})
as well as the promise part of (\ref{erptheruih}). Regarding the
assumption part of (\ref{erptheruih}), we need to prove 
%
\beq
\assp_{\elim{\cgte_1 \para \cgte_2}{p}} &\supseteq& 
\assp_{(\elim{\cgte_1}{p} \para
\elim{\cgte_2}{p})} 
\label {erotihepro}
\eeq
%
where
%
\beqq
\assp_{\elim{\cgte_1 \para \cgte_2}{p}} &=& \forall p\,\bigl(
(\assp_1\cap\assp_2)\cup\complement{(\prom_1\cap\prom_2)}
\bigr)
\\
\assp_{(\elim{\cgte_1}{p} \para
\elim{\cgte_2}{p})} &=& (\forall p\,
\assp_1\cap\forall p\,
\assp_2)\cup\complement{(\exists p\,\prom_1\cap\exists p\,\prom_2)}
\eeqq
%
We have 
%
\beqq
&&
\forall p\,\bigl(
(\assp_1\cap\assp_2)\cup\complement{(\prom_1\cap\prom_2)}
\bigr) 
\\
&\supseteq&
\bigl(\forall p\,(\assp_1\cap\assp_2)\bigr) 
\cup
\bigl(\forall p\,\complement{(\prom_1\cap\prom_2)}\bigr) 
\\
&=&
\bigl(\forall p\,\assp_1\cap
\forall p\,\assp_2\bigr) 
\cup
\complement{\bigl(\exists p\,(\prom_1\cap\prom_2)\bigr)}
\\
&\supseteq&
(\forall p\,
\assp_1\cap\forall p\,
\assp_2)\cup\complement{(\exists p\,\prom_1\cap\exists p\,\prom_2)}
\eeqq
%
which proves (\ref{erotihepro}) and the lemma.
\end{proof}
%
Elimination trivially extends to finite sets of ports, we denote it by 
$\elim{\cgte}{P}$, where $P$ is the considered set of ports.

\subsection{Set of contracts associated to a rich component}
We are now ready to address the case of synchronizing viewpoints when
local ports are shared between viewpoints. More precisely, we shall
formally define what it means to consider a set of contracts
associated to a same rich component.

\begin{definition}[Fusion] \label {sr;otihjeriot}
Let $(\cgte_i)_{i\in I}$ be a finite set of contracts and $Q$ a finite
set of ports. We define \emph{the fusion of $(\cgte_i)_{i\in I}$ with
respect to $Q$} by
%
\beq 
\fusion{(\cgte_i)_{i\in I}}{Q} &\eqdef& \bigmeet_{J\subseteq I}
\bigelim{\,
\|_{j\in J} \cgte_j
\,}{Q}
\label {e;'rotij;i}
\eeq
%
where $J$ ranges over the set of all subsets of $I$.
\end{definition}
%
%
The following particular cases of Definition \ref{sr;otihjeriot} are
of interest:
%
\begin{lemma} \
\begin{enumerate}
\item When $Q=\emptyset$, the fusion reduces to the greatest lower
bound: 
%
\beq 
\fusion{(\cgte_i)_{i\in I}}{\emptyset} &=& \meet_{i\in I}
\cgte_i
\label {rpotuihleui}
\eeq
%
In particular, $\comp\models\fusion{(\cgte_i)_{i\in I}}{\emptyset}$ implies 
$\comp\models\cgte_i$ for each ${i\in I}$.

\item Assume that, for $i=1,2$:
\beq
\assp_i&\supseteq&\prom_1\cap\prom_2
\label {oeirtuheoriu}
\eeq
holds. Then:
\beq
\fusion{(\cgte_i)_{i\in \{1,2\}}}{\emptyset} &= &
\cgte_1\para\cgte_2 
% &=& \cgte_1\meet\cgte_2 
\label {er;otijhpeotie}
\eeq
\item
Assume that, for $i=1,2$:
%
\beq
\forall Q\, (\assp_i\cup\complement{\prom}) &\supseteq&
\forall Q\, (\assp_1\cup\assp_2)
\label {w;otijpeio}
\eeq
%
holds, where $\cgte_1\para\cgte_2=(\assp,\prom)$. Then:
\beq
\fusion{(\cgte_i)_{i\in \{1,2\}}}{Q} &=& \elim{\cgte_1\para\cgte_2}{Q} 
\label {etih;ui}
\eeq
\end{enumerate}
\end{lemma}
Condition (\ref{oeirtuheoriu}) expresses that each rich component is a
valid environment for the other rich components; in other words, the
two contracts are attached to two rich components that together
constitute a valid closed system.
%
Condition (\ref{w;otijpeio}) expresses that the restriction, to $Q$,
of each component is a valid environment for the restriction, to $Q$,
of the other component. This situation corresponds to two rich components
interacting through ports belonging to $Q$, in which ports of $Q$ are
subsequently hidden from outside.
\begin{proof} We successively prove the three statements.
\begin{enumerate}
\item This results immediately from Lemma \ref{wrotheortui}.
\item To prove (\ref{er;otijhpeotie}), note first that the two
expressions only differ by their assumptions, since the promises of
greatest lower bound and parallel composition are identical. Regarding assumptions, let
$\cgte_1\para\cgte_2=(\assp,\prom)$ and
$\cgte_1\meet\cgte_2=(\assp',\prom)$. We have
$\prom=\prom_1\cap\prom_2$ and:
%
\beqq
\assp &=& (\assp_1\cap\assp_2)\cup\complement{\prom}
\\
\assp' &=& (\assp_1\cup\assp_2)
\eeqq
%
From (\ref{oeirtuheoriu}) we get
$\complement{\prom}\supseteq\complement{(\assp_1\cap\assp_2)}$. Therefore,
$\assp=(\assp_1\cap\assp_2)\cup
\complement{\prom}\supseteq(\assp_1\cap\assp_2)\cup
\complement{(\assp_1\cap\assp_2)}=\runs\supseteq\assp'$.
\item 
%
Condition (\ref{w;otijpeio}) implies that 
$
\forall Q\, ((\assp_1\cap\assp_2)\cup\complement{\prom})
\supseteq
\forall Q\, (\assp_1\cup\assp_2)
$. Whence (\ref{etih;ui}) follows.
\end{enumerate}
This proves the lemma.
\end{proof}
The lesson is that fusion boils down to parallel composition for
contracts attached to two different sub-components of a same compound
component, whereas contracts attached to a same component and
involving the same set of ports fuse via the operation of greatest
lower bound.  The general case lies in between and is given by formula
(\ref{e;'rotij;i}).  
%
Finally, the various relations that we have established between
greatest lower bound, parallel composition, and elimination, allows us
to simplify the actual evaluation of the fusion in
general. Corresponding heuristics to guide this remain to be
developed.


%
We are now ready to complete the meaning of Definition
\ref{epfiueipu} for rich components:
%
\begin{definition} [Rich Component, completed] \label {pweifugbepruif}
Let $\richcomp = \bigl(\rcname, \setsofcontracts,
\optimplementation\bigr)$ be a rich component.  Say that
%
\beqq
\optimplementation\models\setsofcontracts &\mbox{iff}&
\optimplementation\models\fusion{(\cgte_i)_{i\in I}}{Q},
\eeqq
%
where $I$ indexes set $\setsofcontracts$, and set $Q$ collects the
ports of $\setsofcontracts$ that are local to $\richcomp$.
\end{definition}

\begin{example}{Running example cont'd: fusion of contracts}
\label {leprifue}

We shall perform a composability study, for the two contracts $\cgte$
and $\cgte'$, and then for their fusion $\fusion{\cgte,\cgte'}{}$.

\paragraph{Study of $\cgte$}
Consider the following two contracts, for the control and monitoring unit,
respectively:
%
\beqq
\varphi = \neg a \wedge x &\mbox{in}&
\left\{\bea{rcl}
\cgte_1 &=& (\,\neg f_1\,,\,[x=a\wedge b]\,)
\\
\cgte_2 &=& (\,\neg \varphi\,,\,\,y=x\,)
\eea\right.
\eeqq
%
Contract $\cgte_1$ of control unit states that, if not faulty, then
the control unit guarantees that $\neg\varphi$ holds, i.e., invariant
$a\vee\neg x$ holds. Contract $\cgte_2$ states that monitoring unit
guarantees that, if not faulty, $y=x$ holds unless $\varphi$ does not
hold.  Putting these two contracts in canonical form and then
computing their fusion yields, by straightforward calculations:
%
\beqq
\cgte_1 &=& (\,\neg f_1\,,\,\neg f_1\Ra[x=a\wedge b]\,)
\nonumber \\
\cgte_2 &=& (\,\neg \varphi \,,\,\neg \varphi \Ra\,y=x\,)
\nonumber \\
\elim{\cgte_1}{x} &=& (\,\neg f_1\,,\,\true\,)
\label {eprogfuiehu}
\\
\elim{\cgte_2}{x} &=& (\,\false\,,\,\true\,)
\label {erpfgouierhpogui}
\\
\elim{\cgte_1 \para \cgte_2}{x} &=& (\,\neg f_1 \wedge P \,,\,
\neg f_1 \Ra[y=a\wedge b]\,) 
\label {erpfiubiu}
\eeqq
%
where $P$ is some predicate (which we don't care of), from which
%
\beqq
\fusion{\cgte_1,\cgte_2}{x}
= \; \elim{\cgte_1}{x} \meet \elim{\cgte_2}{x} \meet \elim{\cgte_1 \para 
\cgte_2}{x} 
\; = \;
\elim{\cgte_1 \para \cgte_2}{x} \; = \; \cgte
\label {perifguehipu}
\eeqq
%
follows, provided that $\cgte$ itself is put in canonical form.


\paragraph{Study of $\cgte'$}


Now, let us focus on the other contract $\cgte'$, by proposing the
following two local contracts, for the control and monitoring units,
respectively:
%
\beqq
\cgte'_1 &=& (\,\false\,,\,\true\,)
\\
\cgte'_2 &=& (\,\neg f_2 \,,\,[y=x\wedge a]\,)
\eeqq
%
The first contract is trivial, and the second one states the invariant
promised if the monitoring unit is not faulty.
%
We first have 
\beq
\mbox{$\elim{\cgte'_1 }{x}=\cgte'_1 $ and 
$\elim{\cgte'_2}{x}=(\,\neg f_2 \,,\,\neg f_2 \Ra\neg\tle\,)$.}
\label {erpofguih}
\eeq
Second, $\prom'_1\cap\prom'_2\,=\,\neg f_2 \Ra[y=x\wedge a]$, whence
\beq
\exists x:(\prom'_1\cap\prom'_2 ) \ = \ \neg f_2 \Ra\neg\tle.
\label {erpfoiuhio}
\eeq
%
Next, 
%
$ 
(\assp'_1\cap\assp'_2)\cup\neg(\prom'_1\cap\prom'_2 )
=
\neg(\prom'_1\cap\prom'_2 )$, which equals
\mbox{$\neg(\neg f_2 \Ra[y=x\wedge a])$,}
%
whence 
%
\beq
\forall x:\left(
(\assp'_1\cap\assp'_2)\cup\neg(\prom'_1\cap\prom'_2 )
\right) &=& \neg(\exists x:(\prom'_1\cap\prom'_2 ))
\nonumber \\
&=& \tle\wedge\neg f_2
\label {pwerfiouwhpfuio}
\eeq
%
Finally, (\ref{erpofguih})--(\ref{pwerfiouwhpfuio}) together prove
that 
%
$
\fusion{\cgte'_1,\cgte'_2}{x} \ = \ \cgte'
$.
%

\paragraph{Study of $\fusion{\cgte,\cgte'}{}$}
The remarkable point is that composability works both across components,
and viewpoints/modes, i.e., we have
%
$
\fusion{\cgte,\cgte'}{} = \fusion{\cgte_1,\cgte_2,\cgte'_1,\cgte'_2}{x}
$.
\end{example}

\subsection{The asymmetric role of ports, a refined theory}
So far we have ignored the role of ports and the corresponding
splitting of responsibilities between the implementation and its
environment, see the discussion in Section~\ref{erogfheri} regarding
this. Such a splitting of responsibilities avoids the competition
between environment and implementation in setting the value of ports and
variables.

\paragraph*{Uncontrolled vs. controlled ports}
Intuitively, an implementation can only provide promises on the value of the
ports it controls.
On ports controlled by the environment, instead, it may only declare
assumptions.
Therefore, we will distinguish between two kinds of ports for
implementations and {\contracts}: those that are \emph{controlled} and those
that are \emph{uncontrolled}.
The latter property is formalized via the following notion of
\emph{receptiveness}:
%
\begin{definition}[Receptiveness] \label {erpthoi}
For $\behav$ an assertion, and $P' \subseteq P$ a subset of its ports,
$\behav$ is said to be $P'$-\emph{receptive} if and only if for all
runs $\sigma'$ restricted to ports belonging to $P'$, there exists a
run in $\sigma$ of $\behav$ such that $\sigma'$ and $\sigma$ coincide
over $P'$.
\end{definition}
%
In words, $\behav$ accepts any history offered to the subset $P'$ of
its ports.  Note that:
%
\begin{lemma} \label {er;'tgijei}
If $E$ is $P'$-receptive, then so is $E\cup E\pprime$ for
any $E\pprime$ having no extra ports or variables as compared to $E$.
\end{lemma}


\paragraph*{Scoping}
% Consider Figure~\ref{pwtfhpefu}. It shows that, i
In some cases, different viewpoints associated with a same rich
component need to interact through some common ports. This motivates
providing a scope for ports, by partitioning them into ports that are
\emph{visible} (outside the underlying component) and ports that are
\emph{local} (to the underlying component).


\paragraph*{Profile}
The two orthogonal classifications controlled vs. uncontrolled and
visible vs. local are collected into a concept of \emph{profile}, for
a set $P$ of ports. A profile is a 4-tuple
$\profile=(\vis,\loc,\uncontrolled,\controlled)$, partitioning $P$ as
$P=\vis\uplus\loc=$ \{visible\}$\uplus$\{local\}, and
$P=\uncontrolled\uplus\controlled=$
\{uncontrolled\}$\uplus$\{controlled\}. Profiles refine as follows:
$\profile \profref \profile' \textrm{ iff } \profile =
\profile'$. Thus profiles form a flat lattice.

\medskip
We are now ready to present our refined theory of contracts, where the
asymmetric role of ports is considered.
\begin{definition}[Implementation]  \label {eotijhroei}
An \emph{implementation} is a pair $M=(\profile,\behav)$, where
$\profile=(\vis,\loc,\uncontrolled,\controlled)$ is a \emph{profile}
over a set $P$ of ports, and $\behav$ is a $\uncontrolled$-receptive
assertion over the set $P$ of ports.
\end{definition}
The last requirement formalizes the fact that an implementation has no
control over the values of ports set by the environment.
%
Implementations refine as follows:
\begin{definition}[Implementation Refinement]\label {pwfuhwpiu}
For $\comp$ and $\comp'$ two implementations, say that $\comp$ refines
$\comp'$, written $\comp \compref \comp'$, if and only if
$\profile\profref\profile'$ and $\behav \subseteq \behav'$.
\end{definition}
%
In defining a parallel composition for implementations, we need to take
into account controlled ports. Each implementation is responsible for
its set of controlled ports, and, in our theory, such responsibility
should not be shared. This motivates the following definition for our
parallel composition of implementations associated with different
rich components (whence the requirement $\loc_1\cap\loc_2=\emptyset$ in
this definition):
%
\begin{definition} [Parallel composition of implementations]
\label {eprotuih}
Let $\comp_1$ and $\comp_2$ be two implementations such that
$\loc_1\cap\loc_2=\emptyset$. Then,  $\comp = \comp_1 \product \comp_2$ is
defined if and only if $\controlled_1 \intersect \controlled_2 =
\emptyset$.  In that case:
\begin{eqnarray*}\bea{rcl}
\vis & = & \vis_1 \union \vis_2 \\
\loc & = & \loc_1 \union \loc_2 
 \\
\controlled & = & \controlled_1 \union \controlled_2 \\
\uncontrolled & = & (\uncontrolled_1 \union \uncontrolled_2) -
(\controlled_1 \union \controlled_2) \\
\behav & = & \behav_1 \times \behav_2.
\eea
\end{eqnarray*}
\end{definition}

\begin{theorem} % [Composition Monotonic]
Implementation composition is monotonic relative to implementation
refinement.
\end{theorem}
\begin{proof}
Since profiles refine via identity, this results boils down to the well known 
monotonicity w.r.t. sets of runs.
\end{proof}


\begin{definition} [Contract] \label {;reouho;e}
  A \emph{contract} is a triple $\cgte=(\profile,\assp,\prom)$, where
$\profile=(\vis,\loc,\uncontrolled,\controlled)$ is a profile over a
set $P$ of ports, and $\assp$ and $\prom$ are two assertions over $P$,
respectively called the \emph{assumptions} and \emph{promises} of
$\cgte$.

Contract $\cgte$ is called \emph{consistent} if $\prom$ is
$\uncontrolled$-receptive, and \emph{compatible} if $\assp$ if
$\controlled$-receptive.
\end{definition}
%
As pointed out in (\ref{erotihjpui}), \emph{contracts are in canonical
form,} meaning that $\prom\supseteq\complement{\assp}$. If this is not
the case, we simply replace $\prom$ by its most permissive version
$\prom\cup\complement{\assp}$, which cannot per se brake consistency, 
thanks to Lemma \ref{er;'tgijei}.

The sets $\assp$ and $\prom$ are not required to be receptive.
However, if $\prom$ is not $\uncontrolled$-receptive, then the promises
constrain the uncontrolled ports of the {\contract}.
This is against our policy of separation of responsibilities, since we
stated that uncontrolled ports should remain entirely under the
responsibility of the environment.
Corresponding {\contracts} are therefore called inconsistent.

\begin{definition} [satisfaction] \label {;oriuihtoe}
  An implementation $\comp$ \emph{satisfies} {\contract} $\cgte$, written
  \mbox{$\comp\models \cgte$}, iff 
$\profile_\comp = \profile_\cgte$ and $\behav_\comp \subseteq \prom_\cgte$.
\end{definition}
By Lemma \ref{er;'tgijei}, if {\contract} $\cgte$ is consistent, then  
$\comp_\cgte\eqdef\prom_\cgte\union\complement{\assp_\cgte}$ is still
the \emph{maximal implementation} satisfying $\cgte$.
%
We now turn to the relation of dominance and its consequences.

\begin{definition} [Contract Dominance] 
\label {prituhpeuirth}
A {\contract} $\cgte = (\profile, \assp, \prom)$ dominates
a {\contract} $\cgte' = (\profile, \assp', \prom')$,
written $\cgte \cgref \cgte'$, if and only if
$\profile=\profile'$,
$\assp \supseteq \assp' $, and 
$\prom \subseteq \prom'$.
\end{definition}

\begin{theorem} [Boolean algebra of contracts] \label {woduygwdvuy}
Let $\cgte_1 = (\profile_1, \assp_1, \prom_1)$ and
$\cgte_2 = (\profile_2, \assp_2, \prom_2)$ be
{\contracts} such that $\profile_1=\profile_2$, we denote it by 
$\profile$.
Then $\cgte = $ \linebreak 
\mbox{$
(\profile, \assp_1 \union \assp_2,
\prom_1 \intersect \prom_2)$} is the greatest
lower bound of $\cgte_1$ and $\cgte_2$, written $\cgte = \cgte_1 \meet
\cgte_2$.
%
Similarly, $\cgte' = (\profile, \assp_1 \intersect
\assp_2, \prom_1 \union \prom_2)$ is the least upper bound of
$\cgte_1$ and $\cgte_2$, written $\cgte = \cgte_1 \meet \cgte_2$.
Finally, the complement of 
$\cgte = (\profile, \assp, \prom)$ is $\complement{\cgte} =
(\profile, \complement{\assp}, \complement{\prom})$.
\end{theorem}
\begin{proof}
This is a direct consequence of Theorem \ref{th:bounds_restr}
% and formulas (\ref{reo;thui},\ref{perithu}).
\end{proof}

Finally, it remains to define the parallel composition of contracts.
Having done this we can directly borrow the definition
\ref{sr;otihjeriot} of fusion, for contracts enhanced with profiles.
%
\begin{definition} [Parallel composition of contracts]
\label {weouirhpeouih}
Let $\cgte_1 = (\profile_1, \assp_1, \prom_1)$ and $\cgte_2 = (\profile_2,
\assp_2, \prom_2)$ be {\contracts}.
The parallel composition, or product, of $\cgte_1$ and $\cgte_2$, written
$\cgte = \cgte_1 \product \cgte_2$, is defined if and only if $\controlled_1
\intersect \controlled_2 = \emptyset$, and in that case is the {\contract}
$\cgte = (\profile, \assp, \prom)$ defined by:
\begin{eqnarray*}\bea{rcl}
\vis & = & \vis_1 \union \vis_2, \\
\loc & = & (\loc_1 \union \loc_2)-(\vis_1 \union \vis_2), \\
\controlled & = & \controlled_1 \union \controlled_2, \\
\uncontrolled & = & (\uncontrolled_1 \union \uncontrolled_2) -
(\controlled_1 \union \controlled_2), \\
\assp & = & (\assp_1 \cap \assp_2) \union \complement{(\prom_1
\cap \prom_2)}, \\
\prom & = & \prom_1 \cap \prom_2.
\eea
\end{eqnarray*}
\end{definition}
\paragraph*{Comments}
First, note that, unlike in
Definition~\ref{eprotuih}, we do not require here that 
$\loc_1 \cap \loc_2=\emptyset$. The reason is that 
we wish to encompass the composition of different viewpoints
attached to a same rich component. (For contracts attached to different
rich components, however, we do have $\loc_1 \cap \loc_2=\emptyset$.)

% Also under composition, assumptions and/or promises may fail to be properly
% receptive, e.g., in case the design contains combinational loops or has
% incompatibilities.
% This should be reported to reveal the incompatibility.

% We kindly suggest the reader revisits the two examples of
% Figures~\ref{priotfuhpeu} and~\ref{pwtfhpefu} with this refined theory.

An important questions is: \textit{is consistency preserved by Boolean
operations or parallel composition?}
% As discussed previously, the assumptions and promises of the bounds
% may at times not be receptive, even if the original assumptions and
% promises were receptive.  Similarly, while it is possible to take the
% complement of a {\contract}, the complement of a receptive set of runs
% may not be receptive.  Hence, the complement {\contract} may be
% inconsistent.  \eproof
% \footnote{We can use mirrors, perhaps, but this require also exchanging the
% roles of controlled and uncontrolled ports when taking the complementation.
% The result is not really a complement, since we can't take the meet or the
% join with the original {\contract}, and therefore verify the condition for
% being a complement.}
% 
% \todo{Procedures to check if a {\contract} is receptive should be proposed
% to verify the consistency of a conjunction of {\contracts}.}
% 
Inconsistency may arise for different reasons.
For example, one obtains an inconsistent {\contract} when taking the greatest
lower bound of two {\contracts}, one of which promises that certain behaviors
will never occur in response to a certain input, while the other one
promises that the remaining behaviors will not occur in response to the same
input (while allowing the first set of behaviors).
Both {\contracts} have legal responses to the input.
But their intersection is empty for the input, thus making the combination
unreceptive.
In this case, inconsistencies is due to two {\contracts} making inconsistent
promises.

Another form of inconsistency may arise when taking parallel composition.
In this case, certain input sequences may be prevented from happening
because they might activate unstable zero-delay feedback loops.
The resulting behaviors may have no representations in our model, thus
resulting in an empty promise.
This problem can be avoided by modeling the oscillating behaviors explicitly
(perhaps using a special value that denotes
oscillation)~\cite{Wolf95Thesis}.
We assume that this kind of inconsistency is taken care of by the user or by
the tools.

The situation with assumptions is different.
Assumptions may become unreceptive as a result of a parallel composition.
This is because the set of controlled ports after a composition is strictly
larger than before.
In particular, ports that were uncontrolled may become controlled, because
they are controlled by the other {\contract}.
In this case, satisfying the assumptions is the responsibility of the other
{\contract}, which acts as an environment.
If the assumptions are not satisfied by the other {\contract}, then the
assumptions of the composition become unreceptive.
That is, a hypothetical environment that wished to prevent a violation of
the assumptions should actually prevent the behavior altogether, something
it cannot do since the port is controlled by one of the {\contract}.
Therefore, unreceptive assumptions denote the existence of an internal
inconsistency within the composition.

Assumptions may also become unreceptive as a result of taking the least
upper bound.
This is a form of inconsistency similar to that of promises when taking the
greatest lower bound.
We do not generally use least upper bounds, so we do not elaborate further
on this situation.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> hrc.tex <==
\section{Heterogeneous Rich Components}\label{sec:hrc}
The main element of our semantic model is a \emph{Heterogeneous Rich
Component}, or simply a component.
A component is composed of an \emph{interface}, its \emph{expected
behavior}, and, optionally, of one or more \emph{implementations}.
The interface of a component consists of a set of ports and flows, which are
used by the component to communicate with the rest of the system and with
the environment.
The expected behavior is instead described by one or several
\emph{assumption}/\emph{promise} pairs, called \emph{contracts}.
Contracts can be combined together using three composition operators:
greatest lower bound, parallel composition and fusion.
The greatest lower bound is used to compose contracts referring to the same
component and which use only variables and flows visible from the
environment.
Parallel composition is used to compute the contract resulting from the
composition of several components.
Fusion generalizes these two operators, and is capable of handling all
cases.
In particular, it is used to compose contracts whenever the greatest lower
bound and parallel composition operators are inappropriate, for instance
when contracts share local variables or flows.
Thus, fusion is the implicit composition of contracts, whenever more than
one contract is attached to a component.
Implementations may be attached to a component, and are usually expressed as
extended state machines, or as host tool models.

We define several relations between components, contracts and
implementations.
\begin{itemize}
  \item The \emph{compatibility} relation relates sets of components.
    It is easier to define the negation of compatibility: A set of
    components are \emph{incompatible} whenever for all environments, at
    least one of the assumption of at least one component is violated.
    This means that in a compatible set of components, the assumption
    resulting from the parallel composition of component contracts is
    universal, i.e., all assumptions required for the correct behavior
    of the system have been discharged.
  \item Contract \emph{dominance} relates assumptions and promises of two
    contracts.
    Contract $\cgte = (\assp, \prom)$ dominates contract $\cgte' = (\assp',
    \prom')$ whenever $\assp' \subseteq \assp$ and $\prom \subseteq \prom'$.
  \item \emph{Satisfaction} relates implementations to contracts.
    An implementation $\comp$ satisfies contract $\cgte = (\assp ,\prom)$
    whenever $\comp \intersect \assp \subseteq \prom$.
  \item \emph{Refinement} relates implementations.  Implementation $\comp$
    refines implementation $\comp'$ whenever $\comp \subseteq \comp'$.
\end{itemize}


==> introduction.tex <==
\section{Introduction}\label{sec:intro}

% NOTICE:
% To better see differences across versions of this file, please follow the
% convention of starting a new line at the end of each period.  By doing so,
% changes will not propagate across sentences, and the output of the diff
% command will be limited to the effective changes in the text.  Thank you!

Embedded systems have emerged as a result of the convergence of information
and communication technology with more traditional engineering sciences and
unconventional domains of application.
A major challenge in the design of these systems is how to make the several
different and heterogeneous formalisms characteristic of such diverse areas
coexist and interact to give a complete view of the design and its
environment.
%One solution is to work at a level of abstraction close to the final
%implementation, where an all-encompassing and expressive model can be used
%to describe complex interactions in considerable details.
%By giving up on abstraction, however, this approach sacrifices the ability
%to apply domain specific techniques for the benefit of integration.
%A host of
Hybrid models with varying degrees of generality have been introduced to
solve this problem~\cite{CarloniPasseronePintoASV06FANDT}.
%solve <-> get around
%especially for domains where safety and the ability to formally analyze the
%system are of primary importance
%More recently,
These techniques have later evolved into metamodeling frameworks,
which are quickly becoming the backbone of modern system level design
methodologies~\cite{BalarinPasseronePintoASV05MEMOCODE,bip,gme,ptolemy,uml_stuff,Rosetta06Book}.
\fixme{Find the appropriate missing references}
In a metamodeling framework, the distinction between the individual% heterogeneous
models is retained throughout the design flow.
By doing so, designers can focus on the distinguishing features of the
subsystems, and apply techniques that rely on specific assumptions about the
models in use.
A typical way to do this is to construct a model of computation that is
general and highly expressive.
This model is individually tailored to the specific needs of each% particular
domain of interest by specializing its operators or by ignoring those
portions of the formalism that are not needed at the level of abstraction
under consideration.
Different models are seen in this framework simply as different
customizations of a common underlying semantic structure.
As the design is refined, the different domains are brought together through
relations that arise from the way each of the models is mapped onto the
common structure, thus relieving the designer from explicitly formulating
the interactions.

In this paper we describe the semantic structure underlying the metamodel
of the SPEEDS integrated project~\cite{speeds}.
SPEEDS is a concerted effort to define the new generation of end-to-end
methodologies, processes and supporting tools for safety-critical embedded
system design.
One of the technical pillars of the SPEEDS approach is the definition of a
semantic-based modeling method that supports the construction of complex
embedded systems by composing heterogeneous subsystems, and that enables the
sound integration of existing and new tools.
At the basis of this approach is the definition of a ``rich-component''
model able to represent functional as well as architectural abstractions,
such as timing, safety and other non-functional performance metrics.
These different viewpoints can be developed separately in the model, and
then integrated and evaluated together in order to derive the most efficient
component-based implementation of the system.

To assist this methodology, SPEEDS is developing a new tool-supported
process, controlled speculative design,
justified by the recent organizational changes and new challenges in
industries such as automotive and aerospace.
Initially organized around large, vertically integrated companies supporting
most of the design in house, the system industry was restructured due to the
emergence of sizeable competitive suppliers.
In this context, OEMs were limited to performing system design and
integration, by importing entire subsystems from suppliers.
This, however, shifted a significant portion of the value to the suppliers,
and eventually resulted in overall lower performance and late errors that
caused delays and excessive additional cost during the system integration
phase.
In the last decade, these industrial sectors went through a profound
reorganization in an attempt to recover value from the supply chain, by
maintaining ownership and focusing on those parts of the design at the core
of their competitive advantage.
The rest of the system was instead centered around standard platforms that
could be developed and shared by otherwise competitors.
Examples of this trend are AUTOSAR in the automotive
industry~\cite{autosar}, and the deployment of Integrated Modular Avionics
(IMA) in aerospace~\cite{ima}.

A lot of effort has been devoted by the research community during the last
years to develop theories and methodologies of component based development
to be used in complex supply chains or OEM/supplier organizations.
The most familiar case is building systems from component libraries.
There, the emphasis is on reuse and adaptation, which is achieved by
exposing a simplified interface of the components, obtained through a
mechanism of abstraction.
When interfaces match, components can be safely composed and deliver the
expected service.
This approach works well for relatively concentrated industries where the
development process is still largely in-house dominated.

When the structure of the supply chain is highly distributed, this approach
is no longer effective, and must be complemented by a precise separation of
responsibilities between the different actors of the OEM/supplier chain.
In SPEEDS, this is accomplished by establishing formal ``contracts'' between
inter- and intra-company design groups.
A contract is a model of a rich component that sets forth the
\emph{assumptions} under which the component may be used by its environment,
and the corresponding \emph{promises} that are guaranteed under such correct
use.
OEMs can use the contract mechanism to define and know precisely what a
given supplier is responsible for, by assigning a specific goal in the form
of a guarantee or promise.
This goal involves only entities the supplier is responsible for.
The other entities involved in the subsystem which are not under the
responsibility of the supplier may still be subject to constraints that are
thus offered to the supplier as assumptions.
Assumptions, however, are under the responsibility of other actors of the
OEM/supplier chain, and can be used by a supplier to satisfy its own
promises.
This design style may include both the functional and non-functional
viewpoints.
This way, designers can more clearly establish and keep track of roles and
responsibilities for the development of the system behavior, as well as for
its deployment onto optimized architectures.

%Since components or sub-systems interact, this implies that each
%entity in the area of interaction must be precisely assigned for
%responsibility to a given supplier, and must remain out of control for
%others.

%This mechanism of assumptions and promises is structured into
%\emph{contracts,} which form the essence of distributed systems
%development involving complex OEM/supplier chains.
%%
%The SPEEDS project focuses on this second type of situation.
%This is why the SPEEDS approach to component based design builts on the
%central concept of {contract.}

%Contracts lead to a notion of compatibility: two components are compatible
%whenever the assumptions of one are satisfied by the guaranteed promises of
%the other.

The semantic foundations that we present in this paper are designed to
support this methodology.
At its basis, the model is a language-based abstraction where composition is
by intersection.
This basic model can then be instantiated to cover functional, timeliness,
safety, and dependability requirements performed across all system design
levels.
In particular, to avoid forcing a specific model of computation, components
in our framework are required to satisfy certain assumptions that guarantee
that different parts of the system may progress at different rates.
\fixme{I'm saying this assuming that we describe, as an example to support
our claims of being a meta-model, the form of a run that includes the
continuous part.}
This is essential for the development of open systems.
On top of the basic model, we build the notion of a contract, which is
central to our methodology, by distinguishing between assumptions and
promises.
Most of the paper will be devoted to developing a compositional theory of
contracts.
The theory includes relations of contract satisfaction and refinement called
dominance, and the derivation of operators for the correct construction of
complete systems.
In addition to the traditional parallel composition, and to enable formal
multi-viewpoint analysis, our model includes boolean meet and join operators
that compute conjunction and disjunction of contracts.
We also introduce a new operator, called fusion, that combines composition
and conjunction to compute the least specific contract that satisfies a set
of specifications, while at the same time taking their interaction into
account.
The differences and the use of these operators are described by several
examples.

In the rest of this paper we will first discuss some related work in
Section~\ref{sec:related}.
Then, we will $\ldots$.
\fxnote{Update this paragraph once the final structure of the paper is
decided}


==> related.tex <==
\section{Related Work}\label{sec:related}
The notion of contract as used in our framework derives from the theory of
abstract data type and was first suggested by Meyer in the context of the
programming language Eiffel~\cite{Meyer92IEEEC}.
In his work, Meyer introduces \emph{preconditions} and \emph{postconditions}
as assertions or specifications for the methods of a class, and
\emph{invariants} for the class itself.
Preconditions correspond to the assumptions under which the method operates,
while postconditions express the promises on the final state of the class at
method termination.
Promises must be guaranteed only if the assumptions are satisfied.
Invariants, on the other hands, are conditions that must be true of the
state of the class regardless of any assumption.
The notion of class inheritance, in this case, is used as a refinement, or
subtyping, relation.
To guarantee safe substitutability, a subclass is only allowed to weaken the
assumptions and to strengthen the promises.

The same idea of distinguishing between assumed and promised conditions was,
in fact, already present in earlier work by Dill, although phrased in less
explicit terms~\cite{Dill89ThesisACM}.
Unlike Meyer, Dill proposes an asynchronous model based on sets of sequences
and parallel composition (trace structures) suitable for hardware, instead
of a model based on state variables and sequential composition, more
suitable for software.
Behaviors (traces) can be either accepted as \emph{successes}, or rejected
as \emph{failures}.
The failures, which are still possible behaviors of the system, correspond
to unacceptable inputs from the environment, and are therefore the
complement of the preconditions.
Because the model is based on behaviors, safe substitutability (or
refinement) is expressed as a conformance order that translates into
conditions of trace containment between the successes and failures of the
specification and the implementation.
A simple analysis shows that the conditions obtained by Dill are equivalent
to requiring that the implementation weaken the assumptions of the
specification while strengthening the promises.
Wolf later extended the same technique to a discrete synchronous
model~\cite{Wolf95Thesis}.
More recently, De Alfaro and Henzinger have proposed Interface Automata
which are similar to synchronous trace structures, where failures are
implicitly all the traces that are not accepted by an automaton representing
the component~\cite{DeAlfaroHenzingerFSE2001}.
Composition is defined on automata, rather than on traces, and requires a
procedure to restrict the state space that is equivalent to the process
called autofailure manifestation of Dill and Wolf.
The authors have also extended the approach to other kinds of behaviors,
including resources and asynchronous behaviors~\cite{resource,permissive}.
A more general approach along the lines proposed by Dill and Wolf is the
work by Negulescu with Process Spaces~\cite{Negulescu98Thesis}, and by
Passerone with Agenta Algebra~\cite{Passerone04Thesis}, both of which extend
the algebraic approach to generic behaviors introduced by
Burch~\cite{Burch92Thesis}.
In both cases, the exact form of the behavior is abstracted, and only the
properties of composition are used to derive general results that apply to
both asynchronous and synchronous models.
An interesting aspect of Process Spaces is the identification of several
derived algebraic operators.
In contrast, Agent Algebra defines the exact relation between concepts such
as parallel composition, refinement and compatibility in the model.

Our notion of contract follows the approach based on concurrent components
which defines assumptions and promises in terms of behaviors, and uses
parallel composition as the main operator for decomposing a design.
This choice is justified by the reactive nature of embedded software, and by
the increasing use of component models that support structured concurrency
as opposed to multi-threaded sequential composition.
In addition, our contracts are intended to be abstract models of a
component, rather than implementations, which, in our context, may
equivalently be done in hardware or software.
Similarly to Process Spaces and Agent Algebra, we develop our theory on the
basis of languages of generic ``runs''.
However, to attain the generality of a metamodel, and to cover
non-functional aspects of the design, we also develop a concrete model
enriched with real-time information that achieves the expressive power of
hybrid systems.
Behaviors are decomponsed into assumptions and promises,
as in Process Spaces, a representation that is more intuitive than, albeit
equivalent to, the one based on the successes and failures of asynchronous
trace structures.
Unlike Process Spaces, however, we explicitly consider inputs and outputs,
which we generalize to the concept of controlled and uncontrolled signals.
This distinction is essential in our framework to determine the exact role
and responsibilities of users and suppliers of components.
This is concretized in our framework by a notion of compatibility which
depends critically on the particular partition of the signals into inputs
and outputs.
We also extend the use of receptiveness of asynchronous trace structures,
which is absent in Process Spaces, to define formally the condition of
compatibility of components for open systems.

Our refinement relation between contracts, which we call \emph{dominance} to
distinguish it from refinement between implementations of the contracts,
follows the usual scheme of weakening the assumption and strengthening the
guarantees.
The order induces boolean operators of conjunction and disjunction, which
resembles those of asynchronous trace structures and Process Spaces.
In addition, we also define a \emph{fusion} operator that combines the
operation of composition and conjunction for a set of contracts.
This operator is introduced to make it easier for the user to express the
interaction between contracts related to different viewpoints of a
component.

The model that we present in this paper is based on execution traces, and is
therefore inherently limited to representing linear time properties.
In other words, the branching structure of a process whose semantics is
expressed in our model is abstracted, and the exact state in which
non-deterministic choices are taken is lost.
Despite this, the equivalence relation that is induced by our notion of
dominance between contracts is more distinguishing than the traditional
trace containment used when executions are not partitioned between
assumptions and promises.
\fxnote{Any good reference for trace containment?}
This was already observed by Dill, with the classic example of the vending
machine~\cite{Dill89ThesisACM}.
The situation is also similar to that described by Brookes et al.\ in CSP
using refusal sets~\cite{BrookesHoareRoscoe84JACM}.
There, every accepted sequence of actions is complemented by the set of
possible \emph{refusals}, i.e., by the set of actions that may not be
accepted after executing that particular sequence.
Equivalence is then defined as equality of sequences with their refusal
sets.
Under these definitions, it is shown that the resulting equivalence is
stronger than trace equivalence (equality of trace sets), but weaker than
observation equivalence~\cite{Engelfriet,Brookes83ICALP}.
One can set up a bijection between our model and the model based on refusal
sets.
However, a precise characterization of the exact relationships with our
model, in particular with reagrd to the notion of composition, is deferred
for our future work.



While component-based design has proven successful in software development,
achieving productivity boosts by re-use, the design of complex embedded
systems requires component models covering the complete spectrum of
non-functional constraints, such as timing, dependability, safety, resource
consumptions, and so on.
SPEEDS rich components go beyond the expressive power of pertinent UML
profiles or Autosar's components model so as to support realizability
analysis of non-functional constraints already at system- and/or
function-network specification time, while supporting the complete design
cycle to deployed components.

